Delocalisation and continuity in 2D: loop O(2), six-vertex, and random-cluster models

We prove the existence of macroscopic loops in the loop O(2) model with $\frac12\leq x^2\leq 1$ or, equivalently, delocalisation of the associated integer-valued Lipschitz function on the triangular lattice. This settles one side of the conjecture of Fan, Domany, and Nienhuis (1970s-80s) that $x^2 = \frac12$ is the critical point. We also prove delocalisation in the six-vertex model with $0<a,\,b\leq c\leq a+b$. This yields a new proof of continuity of the phase transition in the random-cluster and Potts models in two dimensions for $1\leq q\leq 4$ relying neither on integrability tools (parafermionic observables, Bethe Ansatz), nor on the Russo-Seymour-Welsh theory. Our approach goes through a novel FKG property required for the non-coexistence theorem of Zhang and Sheffield, which is used to prove delocalisation all the way up to the critical point. We also use the $\mathbb T$-circuit argument in the case of the six-vertex model. Finally, we extend an existing renormalisation inequality in order to quantify the delocalisation as being logarithmic, in the regimes $\frac12\leq x^2\leq 1$ and $a=b\leq c\leq a+b$. This is consistent with the conjecture that the scaling limit is the Gaussian free field.

==> sections/00_abstract_arxiv.tex <==
We prove the existence of macroscopic loops in the loop O(2) model with
$\frac12\leq x^2\leq 1$ or, equivalently, delocalisation of the associated
integer-valued Lipschitz function on the triangular lattice. This settles one
side of the conjecture of Fan, Domany, and Nienhuis (1970s--80s) that $x^2 =
\frac12$ is the critical point.

We also prove delocalisation in the six-vertex model with $0<a,b\leq c\leq a+b$.
This yields a new proof of continuity of the phase transition in the
random-cluster and Potts models in two dimensions for $1\leq q\leq 4$ relying
neither on integrability tools (parafermionic observables, Bethe Ansatz), nor on
the Russo-Seymour-Welsh theory.

Our approach goes through a novel FKG property required for the non-coexistence
theorem of Zhang and Sheffield, which is used to prove delocalisation all the
way up to the critical point.  We also use the $\mathbb T$-circuit argument in
the case of the six-vertex model.

Finally, we extend an existing renormalisation inequality in order to quantify
the delocalisation as being logarithmic, in the regimes $\frac12\leq x^2\leq 1$
and $a=b\leq c\leq a+b$.  This is consistent with the conjecture that the
scaling limit is the Gaussian free field.


==> sections/OLD_preface.tex <==

\subsection{Preface}

Broadly speaking, we consider integer-valued height functions on two-dimensional lattices.
Height functions have a phase transition called the \emph{localisation-delocalisation transition};
the phase indicates whether or not the variance of the height at a fixed vertex grows infinite as the
boundary is taken further and further away.
This phase transition is known to coincide with several other important phase transitions
in 2D statistical mechanics, for example:
\begin{itemize}
	\item The continuity-discontinuity transition in the 2D Fortuin--Kasteleyn (FK) percolation model
	coincides with the delocalisation transition in
	the corresponding six-vertex model~\cite{DumSidTas17,DumGagHar16,GlaPel19,Lis21},
	\item The Berezinskii--Kosterlitz--Thouless (BKT) transition in the XY model coincides
	with the delocalisation transition in the dual height function (which is more or less equivalent to the discrete Gaussian model)~\cite{LisEng23elementary,Aiz21,Lam23,LisEng23dual}.
\end{itemize}
The analysis of height functions is important for these reasons and because it
describes how symmetries of 2D lattice models are (not) broken.

There exist several strategies to prove height function delocalisation,
such as for example:
Coulomb gas expansions~\cite{FroSpe81}, explicit calculations~\cite{Kenyon01},
the Bethe Ansatz~\cite{DumKarManOul20}, and parafermionic observables~\cite{DumGlaPel21,Lis21}.


Sheffield, who was the first to systematically use percolation theory
for the analysis of height function, used the non-coexistence theorem to prove
that localisation can only occur at slopes which lie in a certain lattice~\cite{She05}.
It was later observed that this approach can actually be used to prove height function delocalisation,
in the work of Chandgotia, Peled, Sheffield, and Tassy who proved delocalisation of the uniform six-vertex model~\cite{ChaPelSheTas21}.
Around the same time, Manolescu and the first author proved height function delocalisation
for the uniform Lipschitz function on the triangular lattice, by applying Zhang's argument
to a spin representation of the height function~\cite{GlaMan21}.
The second author recently used the non-coexistence theorem to derive delocalisation for general
height functions on the hexagonal lattice~\cite{Lam22deloc}.

The first contribution of this article consists in a delocalisation proof for
the loop~\O{2} and six-vertex models, going all the way up to the (conjectured) critical point,
and using directly the non-coexistence theorem.
For the loop~\O{2} model this generalises~\cite{GlaMan21} and~\cite{DumGlaPel21};
for the six-vertex model this yields a new proof complementary to the recent
breakthrough work of Duminil-Copin, Karrila, Manolescu, and Oulamara~\cite{DumKarManOul20}.
In our proofs the non-coexistence theorem is applied to a two-spin representation of each model,
which in turn has been introduced in~\cite{GlaMan21} for the loop model and in~\cite{Lis21}
for the six-vertex model.
Using the Baxter--Kelland--Wu coupling which relates the six-vertex model to the random-cluster model~\cite{BaxKelWu76},
we then argue that delocalisation implies continuity of the phase transition on the random-cluster side
for the cluster weight $1\leq q\leq 4$,
thus providing a new proof complementary to~\cite{DumSidTas17}
(that relies on the parafermionic observable).
This implication is the reverse of the strategy in~\cite{Lis21},
and yields a new route to continuity that does not rely on the application of
integrability arguments, which are understood to be extremely powerful yet
less probabilistic in spirit.
This is the second contribution of this article.

As effective as the non-coexistence theorem is in deriving this result,
it has limitations when it comes to deriving quantitative information.
A general strategy to derive quantitative percolation results
from qualitative input on the phase transition
was developed in~\cite{DumSidTas17}.
In that article,
Duminil-Copin, Sidoravicius, and Tassion introduce the \emph{renormalisation inequality}
which yields a dichotomy for the quantitative behaviour of the system.
This strategy was first implemented by Manolescu and the first author in the context of height functions to \emph{quantify}
the delocalisation, namely, they proved that the variance grows logarithmically
in the distance to the boundary of the domain~\cite{GlaMan21}.
This is significant because the logarithm indicates that each scale contributes a unit of variance.
As a third contribution, we extend this renormalisation inequality to the height
functions in this article, which implies that the delocalisation is also logarithmic.



==> sections/loop/conclusions.tex <==
\subsection{Proof of Theorems~\ref{thm:loop_soft_deloc} and~\ref{thm:soft_Lip_deloc}}

An additional ingredient that holds only when~$1/\sqrt{2} \leq x \leq 1$ is the duality relation~\eqref{eq:super_duality}.
The next proposition shows that how it implies ergodicity in~$\sigma^\white$ and existence of infinitely many loops around any given face.

\begin{proposition}\label{prop:ergo-lip}
	Let~$1/\sqrt{2} \leq x \leq 1$. Then, $\muSpin_x^\blackp$ is ergodic and
	\[
		\muSpin_x^\blackp(\text{each face is surrounded by infinitely many black loops}) = 1.
	\]
\end{proposition}

\begin{proof}
	By Proposition~\ref{prop:inf-vol-lip}, the marginal of~$\muSpin_x^\blackp$ on~$\xi^\blackp$ is ergodic and translation invariant with respect to isometries of~$\upvert(\hexlattice)$.
	In addition, taking a limit over finite domains in Lemma~\ref{lemma:loop_rhombus_crossing}, we obtain, for every~$m\geq 1$,
	\[
		\muSpin_x^\blackp(\calH_m(\xi^\blackp)) \geq \tfrac14.
	\]
	Thus, the general Russo--Seymour--Welsh theory developed by Tassion~\cite{Tas16} applies and
	\[
		\muSpin_x^\blackp(\text{each face is surrounded by infinitely many circuits of } \xi^\blackp) = 1.
	\]	
	In particular, all connected components of $Y(\xi^\black)^*$ are bounded and hence the marginal of~$\muSpin_x^\blackp$ on~$\sigma^\white$ is ergodic.
	
	Thus, the marginal of~$\muSpin_x^\blackp$ on~$\sigma^\white$ is ergodic and satisfies the finite energy property and the FKG inequality.
	It is then standard that Burton--Keane and Zhang's arguments exclude coexistence of infinite clusters of white pluses and of white minuses.
	By symmetry of~$\muSpin_x^\blackp$ with respect to a global spin flip in~$\sigma^\white$, we then obtain
	\[
		\muSpin_x^\blackp(\text{neither } \{\sigma^\white=+\} \text{ nor } \{\sigma^\white=-\} \text{ contains an infinite cluster}) = 1.
	\]
	Hence, each face is surrounded by infinitely many white loops almost surely.
	The statement then follows, since the colour of each loop is black or white with equal probability.
\end{proof}

\begin{remark}
	We mention a beautiful recent work of K\"ohler-Schindler and Tassion~\cite{KohTas20} that strengthens the statement of~\cite{Tas16}.
	While it gives better bounds on the behaviour of~$\xi^\blackp$ (circuits appear at every scale), unfortunately this does not imply logarithmic delocalisation and in general does not shorten our proofs.
\end{remark}

We are not ready to finish the proofs of Theorems~\ref{thm:loop_soft_deloc} and~\ref{thm:soft_Lip_deloc}.

\ag{Continue here}

\begin{proof}[Proof of Theorem~\ref{thm:loop_soft_deloc}]	
	Finally, the above implies that~$\muSpin_x^{r+}$-a.s. every face is surrounded by infinitely many circuits of~$\xi^\blackm$.
	By FKG inequality, this implies that, for any sequence of domains~$\domain_k\nearrow \H$, the marginals of~$\muSpin_{\domain_k,x}^{r-}$ on~$\sigma^\black,\xi^\black$ converge to the marginal of~$\muSpin_x^{r+}$.
	Then, the same also holds for the marginal of~$\muSpin_{\domain_k,x}$ on~$\sigma^\black,\xi^\black$ since it is stochastically between~$\muSpin_{\domain_k,x}^{r-}$ and~$\muSpin_{\domain_k,x}^{r+}$.
	As in Lemma~\ref{lem:lip-joint}, we get that the joint distributions~$\muSpin_{\domain_k,x}$ of~$\sigma^\black,\sigma^\white$ converge to~$\muSpin_x^{r+}$.
	By~\eqref{eq:loops-to-spins}, the marginal of~$\muSpin_{\domain_k,x}$ on~$\omega_r\cup\omega_b$ coincides with~$\muLoop_{\domain_k,2,x}$ and, by the above, converges to the marginal of~$\muSpin_x^{r+}$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:soft_Lip_deloc}]
	Given a loop configuration~$\omega$ sampled from~$\muLoop_{\domain,2,x}$, we define a Lipschitz function~$h$ as follows: it is fixed to be~$0$ at boundary faces; the value of~$h$ is constant along on clusters of~$\omega^*$; when two clusters are separated by a loop, the value of~$h$ is bigger (resp. smaller) by~$1$ at the inner cluster if the loop is oriented clockwise (resp. counter-clockwise).
	It is easy to check that!$h$ is well-defined and its law is exactly~$\muLip_{\domain,x}$.
	Moreover, by the construction
	\[
		\mathrm{Var}_{\domain,x} [h] = \E_{\domain,2,x}[\omega].
	\]
	By Theorem~\ref{thm:loop}, the right-hand side diverges as the domain becomes bigger and bigger.
\end{proof}


\ag{The text below was copied. Here we should prove uniqueness of the Gibbs measure for the loop \O{2} model.}

The previous result implies that the law of $\omega[h]$
in $\muLip_{\domain_n,x}^{01}$
converges to some limit $\nu$ in the weak topology,
in which each face is $\nu$-almost surely surrounded by infinitely many $\omega$-loops.
By a standard coupling argument for height functions,
this implies that the distribution of $\omega[h]$ in $\muLip_{\domain_n,x}^0$
also converges to $\nu$.
This limit $\nu$ is the unique Gibbs measure for the original loop \O{2} model.

